DKVF: A Framework for Rapid Prototyping and Evaluating Distributed Key-value Stores

We present our framework DKVF that enables one to quickly prototype and evaluate new protocols for key-value stores and compare them with existing protocols based on selected benchmarks. Due to limitations of CAP theorem, new protocols must be developed that achieve the desired trade-off between consistency and availability for the given application at hand. Hence, both academic and industrial communities focus on developing new protocols that identify a different (and hopefully better in one or more aspect) point on this trade-off curve. While these protocols are often based on a simple intuition, evaluating them to ensure that they indeed provide increased availability, consistency, or performance is a tedious task. Our framework, DKVF, enables one to quickly prototype a new protocol as well as identify how it performs compared to existing protocols for pre-specified benchmarks. Our framework relies on YCSB (Yahoo! Cloud Servicing Benchmark) for benchmarking. We demonstrate DKVF by implementing four existing protocols --eventual consistency, COPS, GentleRain and CausalSpartan-- with it. We compare the performance of these protocols against different loading conditions. We find that the performance is similar to our implementation of these protocols from scratch. And, the comparison of these protocols is consistent with what has been reported in the literature. Moreover, implementation of these protocols was much more natural as we only needed to translate the pseudocode into Java (and add the necessary error handling). Hence, it was possible to achieve this in just 1-2 days per protocol. Finally, our framework is extensible. It is possible to replace individual components in the framework (e.g., the storage component).

==> engine.tex <==
\section{Storage Engine Configuration}
\label{sec:engine}

\name comes with a driver for Oracle Berkeley-DB as its default storage engine. We believe the default storage is sufficient for most prototyping purposes. There are cases, however, we may want to use another product for our underlying storage. For instance, if we want to compare our protocol with another system based on a storage system other than Berkeley-DB. We can integrate any storage engine with \name by writing a driver for it. The driver must extend class \code{Storage}. The interface of \code{Storage} is very minimal, and only requires basic \code{put (key, value)} and \code{get (key)} operations. We can, however, add any operation that we want, and use it in our protocol layer. %To do that, we only need to call \code{getStorage()} method of the \code{DKVFServer} or \code{DKVFClient} classes, and cast it to our desired driver. We now can call any method of the driver. 

\subsection{Data Replication and Storage Engine}
Regarding the storage, an important question is which layer is responsible for data replication? There are two options for data replication:  1) the protocol does the replication, 2) the storage engine does the replication. We refer to the first option demonstrated in Figure \ref{fig:dbArch1} as \textit{server centric} configuration, while we refer to the second option demonstrated in Figure \ref{fig:dbArch2} as \textit{storage centric} configuration. The default storage of \name is server centric: the storage is provided by Berkeley-DB in each node, but storage layer does not replicate data automatically. Instead, the protocol designer needs to implement replication by sending replicate messages. Server centric configuration is more flexible, as the protocol designer can easily choose any replication strategy that suites the protocol the best.
\begin{figure} 
\begin{center}
\includegraphics[scale=0.32]{figs/dbArch1}
\caption{The architecture of server centric storage engine configuration}
\label{fig:dbArch1}
\end{center}
\end{figure}


We can, however, totally delegate the replication to the storage engine, and only focus on consistency on the higher level. This approach is the same as \textit{bolt-on} consistency  approach proposed in []. An important advantage of this method is that the protocol designer does not need to manage data replication, and it is done by the storage. However, it reduces the flexibility, as different products have their own replication strategy. Thus, if we delegate replication to storage engine, we have to accept that strategy, even if that strategy is not the best choice for our protocol. For instance, Dynamo [] assumes nodes in a circle. Each node replicates its data in next two nodes in the circle. This replication strategy is not compatible with full replication policy used in protocols such as [cops][gentlerain][causalSpartan]. 




\begin{figure} 
\begin{center}
\includegraphics[scale=0.32]{figs/dbArch2}
\caption{The architecture of storage centric storage engine configuration}
\label{fig:dbArch2}
\end{center}
\end{figure}

